Embedding a Deterministic BFT Protocol in a Block DAG

This work formalizes the structure and protocols underlying recent distributed systems leveraging block DAGs, which are essentially encoding Lamport's happened-before relations between blocks, as their core network primitives. We then present an embedding of any deterministic Byzantine fault tolerant protocol $\mathcal{P}$ to employ a block DAG for interpreting interactions between servers. Our main theorem proves that this embedding maintains all safety and liveness properties of $\mathcal{P}$. Technically, our theorem is based on the insight that a block DAG merely acts as an efficient reliable point-to-point channel between instances of P while also using $\mathcal{P}$ for efficient message compression.

==> pics/block-dag-brdcst-b2.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{green}{rgb}{0,1,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \node[ipe node]
     at (32, 752) {$s_1$};
  \node[ipe node]
     at (32, 680) {$s_2$};
  \draw[{<[ipe arrow tiny]}-]
    (224, 764)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw
    (48, 768) rectangle (208, 720);
  \node[ipe node]
     at (52, 756) {$B_1$};
  \draw[{<[ipe arrow tiny]}-]
    (424, 760)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[shift={(224, 768)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (228, 756) {$B_2$};
  \node[ipe node, font=\footnotesize]
     at (228, 740) {$\ghost{%
\inm = \varnothing}$};
  \node[ipe node, font=\footnotesize]
     at (228, 728) {$\ghost{%
\outm = (\ell_2, \ECHO\ r_2)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[shift={(224, 704)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (228, 692) {$B_{3}$};
  \node[ipe node]
     at (32, 616) {$s_3$};
  \draw[shift={(224, 640)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (228, 628) {$B_4
$};
  \node[ipe node]
     at (32, 552) {$s_4$};
  \draw[shift={(224, 576)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (228, 564) {$B_5$};
  \draw[shift={(424, 768)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (428, 756) {$B_6$};
  \node[ipe node, font=\footnotesize]
     at (428, 740) {$\ghost{%
\inm = (\ell_2, \ECHO\ r_2)\ \From\ \{s_1 \}}$};
  \node[ipe node, font=\footnotesize]
     at (428, 728) {$\ghost{%
\outm = (\ell_2, \ECHO\ r_2)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[shift={(424, 704)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (428, 692) {$B_{7}$};
  \node[ipe node, font=\footnotesize]
     at (428, 676) {$\ghost{%
\inm =(\ell_2, \ECHO\ r_2)\ \From\ \{s_1 \}}$};
  \node[ipe node, font=\footnotesize]
     at (428, 664) {$\ghost{%
\outm = (\ell_2, \ECHO\ r_2)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[shift={(424, 640)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (428, 628) {$B_8$};
  \draw[-{>[ipe arrow tiny]}]
    (208, 720)
     -- (224, 640);
  \draw[-{>[ipe arrow tiny]}]
    (208, 720)
     -- (224, 704);
  \draw[-{>[ipe arrow tiny]}]
    (208, 716)
     -- (224, 576);
  \draw[-{>[ipe arrow tiny]}]
    (384, 692)
     -- (424, 740);
  \draw[-{>[ipe arrow tiny]}]
    (380, 640)
     -- (424, 728);
  \draw[{<[ipe arrow tiny]}-]
    (424, 680)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[{<[ipe arrow tiny]}-]
    (424, 620)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[-{>[ipe arrow tiny]}]
    (384, 732)
     -- (424, 696);
  \draw[-{>[ipe arrow tiny]}]
    (384, 628)
     -- (424, 668);
  \draw[-{>[ipe arrow tiny]}]
    (384, 552)
     -- (424, 604);
  \draw[-{>[ipe arrow tiny]}]
    (384, 672)
     -- (424, 636);
  \draw[{<[ipe arrow tiny]}-]
    (624, 760)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[shift={(624, 768)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (628, 756) {$B_9$};
  \node[ipe node, font=\footnotesize]
     at (628, 740) {$\ghost{%
\inm = (\ell_2, \ECHO\ r_2)\ \From\ \{s_1, s_2 \}}$};
  \node[ipe node, font=\footnotesize]
     at (628, 728) {$\ghost{%
\outm = \varnothing}$};
  \draw[shift={(624, 704)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (628, 692) {$B_{10}$};
  \node[ipe node, font=\footnotesize]
     at (628, 676) {$\ghost{%
\inm = (\ell_2, \ECHO\ r_2)\ \From\ \{s_1, s_2 \}}$};
  \node[ipe node, font=\footnotesize]
     at (628, 664) {$\ghost{%
\outm = \varnothing}$};
  \draw[shift={(624, 640)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (628, 628) {$B_{11}$};
  \node[ipe node, font=\footnotesize]
     at (628, 612) {$\ghost{%
\inm = (\ell_2, \ECHO\ r_2)\ \From\ \{s_1, s_2 \}}$};
  \node[ipe node, font=\footnotesize]
     at (628, 600) {$\ghost{%
\outm = (\ell_2, \ECHO\ r_2)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[-{>[ipe arrow tiny]}]
    (584, 692)
     -- (624, 740);
  \draw[-{>[ipe arrow tiny]}]
    (580, 640)
     -- (624, 728);
  \draw[{<[ipe arrow tiny]}-]
    (624, 680)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[{<[ipe arrow tiny]}-]
    (624, 620)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[-{>[ipe arrow tiny]}]
    (584, 732)
     -- (624, 696);
  \draw[-{>[ipe arrow tiny]}]
    (584, 628)
     -- (624, 668);
  \draw[-{>[ipe arrow tiny]}]
    (580, 720)
     -- (624, 604);
  \draw[-{>[ipe arrow tiny]}]
    (584, 672)
     -- (624, 636);
  \draw[shift={(48, 704)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \draw[shift={(48, 640)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \draw[shift={(48, 576)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \draw[{<[ipe arrow tiny]}-]
    (224, 560)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (224, 620)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (224, 680)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \node[ipe node]
     at (112, 776) {$k_1$};
  \node[ipe node]
     at (288, 776) {$k_2$};
  \node[ipe node]
     at (504, 776) {$k_3$};
  \node[ipe node]
     at (688, 776) {$k_4$};
\end{tikzpicture}


==> pics/block-dag-brdcst.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{green}{rgb}{0,1,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \node[ipe node]
     at (32, 752) {$s_1$};
  \node[ipe node]
     at (32, 680) {$s_2$};
  \draw[{<[ipe arrow tiny]}-]
    (224, 764)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw
    (48, 768) rectangle (208, 720);
  \node[ipe node]
     at (52, 756) {$B_1$};
  \node[ipe node, font=\footnotesize]
     at (52, 740) {$\ghost{%
\inm = \varnothing}$};
  \node[ipe node, font=\footnotesize]
     at (52, 728) {$\ghost{%
\outm = (\ell_1, \ECHO\ r_1)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[{<[ipe arrow tiny]}-]
    (424, 760)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[shift={(224, 768)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (228, 756) {$B_2$};
  \node[ipe node, font=\footnotesize]
     at (228, 740) {$\ghost{%
\inm =  (\ell_1, \ECHO\ r_1)\ \From\ \{s_1 \}}$};
  \node[ipe node, font=\footnotesize]
     at (228, 728) {$\ghost{%
\outm =  (\ell_1, \ECHO\ r_1)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[shift={(224, 704)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (228, 692) {$B_{3}$};
  \node[ipe node, font=\footnotesize]
     at (228, 676) {$\ghost{%
\inm =  (\ell_1, \ECHO\ r_1)\ \From\ \{s_1 \}}$};
  \node[ipe node, font=\footnotesize]
     at (228, 664) {$\ghost{%
\outm = (\ell_1, \ECHO\ r_1)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \node[ipe node]
     at (32, 616) {$s_3$};
  \draw[shift={(224, 640)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (228, 628) {$B_4
$};
  \node[ipe node, font=\footnotesize]
     at (228, 612) {$\ghost{%
\inm =  (\ell_1, \ECHO\ r_1)\ \From\ \{s_1 \}}$};
  \node[ipe node, font=\footnotesize]
     at (228, 600) {$\ghost{%
\outm =  (\ell_1, \ECHO\ r_1)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \node[ipe node]
     at (32, 552) {$s_4$};
  \draw[shift={(224, 576)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (228, 564) {$B_5$};
  \node[ipe node, font=\footnotesize]
     at (228, 548) {$\ghost{%
\inm =  (\ell_1, \ECHO\ r_1)\ \From\ \{s_1 \}}$};
  \node[ipe node, font=\footnotesize]
     at (228, 536) {$\ghost{%
\outm =  (\ell_1, \ECHO\ r_1)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[shift={(424, 768)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (428, 756) {$B_6$};
  \node[ipe node, font=\footnotesize]
     at (428, 740) {$\ghost{%
\inm = (\ell_1, \ECHO\ r_1)\ \From\ \{s_1, s_2, s_3 \}}$};
  \node[ipe node, font=\footnotesize]
     at (428, 728) {$\ghost{%
\outm = (\ell_1, \READY\ r_1)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[shift={(424, 704)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (428, 692) {$B_{7}$};
  \node[ipe node, font=\footnotesize]
     at (428, 676) {$\ghost{%
\inm = (\ell_1, \ECHO\ r_1)\ \From\ \{s_1, s_2, s_3 \}}$};
  \node[ipe node, font=\footnotesize]
     at (428, 664) {$\ghost{%
\outm = (\ell_1, \READY\ r_1)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[shift={(424, 640)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (428, 628) {$B_8$};
  \node[ipe node, font=\footnotesize]
     at (428, 612) {$\ghost{%
\inm = (\ell_1, \ECHO\ r_1)\ \From\ \{s_2, s_3, s_4 \}}$};
  \node[ipe node, font=\footnotesize]
     at (428, 600) {$\ghost{%
\outm = (\ell_1, \READY\ r_1)\ \To\ \{s_1, s_2, s_3, s_4 \}}$};
  \draw[-{>[ipe arrow tiny]}]
    (208, 720)
     -- (224, 640);
  \draw[-{>[ipe arrow tiny]}]
    (208, 720)
     -- (224, 704);
  \draw[-{>[ipe arrow tiny]}]
    (208, 720)
     -- (224, 576);
  \draw[-{>[ipe arrow tiny]}]
    (384, 692)
     -- (424, 740);
  \draw[-{>[ipe arrow tiny]}]
    (380, 640)
     -- (424, 728);
  \draw[{<[ipe arrow tiny]}-]
    (424, 680)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[{<[ipe arrow tiny]}-]
    (424, 620)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[-{>[ipe arrow tiny]}]
    (384, 732)
     -- (424, 696);
  \draw[-{>[ipe arrow tiny]}]
    (384, 628)
     -- (424, 668);
  \draw[-{>[ipe arrow tiny]}]
    (384, 552)
     -- (424, 604);
  \draw[-{>[ipe arrow tiny]}]
    (384, 672)
     -- (424, 636);
  \draw[{<[ipe arrow tiny]}-]
    (624, 760)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[shift={(624, 768)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (628, 756) {$B_9$};
  \node[ipe node, font=\footnotesize]
     at (628, 740) {$\ghost{%
\inm = (\ell_1, \READY\ r_1)\ \From\ \{s_1, s_2, s_3 \}}$};
  \node[ipe node, font=\footnotesize]
     at (628, 728) {$\ghost{%
\outm = \varnothing}$};
  \draw[shift={(624, 704)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (628, 692) {$B_{10}$};
  \node[ipe node, font=\footnotesize]
     at (628, 676) {$\ghost{%
\inm = (\ell_1, \READY\ r_1)\ \From\ \{s_1, s_2, s_3 \}}$};
  \node[ipe node, font=\footnotesize]
     at (628, 664) {$\ghost{%
\outm = \varnothing}$};
  \draw[shift={(624, 640)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \node[ipe node]
     at (628, 628) {$B_{11}$};
  \node[ipe node, font=\footnotesize]
     at (628, 612) {$\ghost{%
\inm =(\ell_1, \READY\ r_1)\ \From\ \{s_1, s_2, s_3 \}}$};
  \node[ipe node, font=\footnotesize]
     at (628, 600) {$\ghost{%
\outm = \varnothing}$};
  \draw[-{>[ipe arrow tiny]}]
    (584, 692)
     -- (624, 740);
  \draw[-{>[ipe arrow tiny]}]
    (580, 640)
     -- (624, 728);
  \draw[{<[ipe arrow tiny]}-]
    (624, 680)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[{<[ipe arrow tiny]}-]
    (624, 620)
     arc[start angle=50.1944, end angle=129.8056, radius=31.241];
  \draw[-{>[ipe arrow tiny]}]
    (584, 732)
     -- (624, 696);
  \draw[-{>[ipe arrow tiny]}]
    (584, 628)
     -- (624, 668);
  \draw[-{>[ipe arrow tiny]}]
    (580, 720)
     -- (624, 604);
  \draw[-{>[ipe arrow tiny]}]
    (584, 672)
     -- (624, 636);
  \draw[shift={(48, 704)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \draw[shift={(48, 640)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \draw[shift={(48, 576)}, xscale=1.1429]
    (0, 0) rectangle (140, -48);
  \draw[{<[ipe arrow tiny]}-]
    (224, 560)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (224, 620)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (224, 680)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \node[ipe node]
     at (112, 776) {$k_1$};
  \node[ipe node]
     at (288, 776) {$k_2$};
  \node[ipe node]
     at (504, 776) {$k_3$};
  \node[ipe node]
     at (688, 776) {$k_4$};
\end{tikzpicture}


==> pics/byz-duplicate.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \node[ipe node]
     at (44, 788) {$\byz{s}$};
  \node[ipe node]
     at (44, 760) {$s$};
  \draw[{<[ipe arrow tiny]}-]
    (132, 796)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (140, 780)
     -- (116, 768);
  \draw[shift={(64, 799.999)}, xscale=1.0833, yscale=0.8333]
    (0, 0) rectangle (48, -24);
  \draw[shift={(132, 799.999)}, xscale=1.0833, yscale=0.8333]
    (0, 0) rectangle (48, -24);
  \node[ipe node]
     at (68, 760) {$B$};
  \draw[shift={(64, 771.999)}, xscale=1.0833, yscale=0.8333]
    (0, 0) rectangle (48, -24);
  \node[ipe node]
     at (148, 808) {$1$};
  \node[ipe node]
     at (80, 808) {$0$};
  \draw[{<[ipe arrow tiny]}-]
    (100, 780)
     -- (100, 772);
\end{tikzpicture}


==> pics/byz-equviocating-same-attestant.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \node[ipe node]
     at (44, 788) {$s$};
  \node[ipe node]
     at (44, 760) {$\byz{s}$};
  \draw[{<[ipe arrow tiny]}-]
    (132, 796)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (140, 780)
     -- (132, 764);
  \draw[shift={(64, 799.999)}, xscale=1.0833, yscale=0.8333]
    (0, 0) rectangle (48, -24);
  \draw[shift={(132, 799.999)}, xscale=1.0833, yscale=0.8333]
    (0, 0) rectangle (48, -24);
  \node[ipe node]
     at (68, 760) {$B$};
  \draw[shift={(64, 771.999)}, xscale=1.0833, yscale=0.8333]
    (0, 0) rectangle (48, -24);
  \node[ipe node]
     at (148, 808) {$1$};
  \node[ipe node]
     at (80, 808) {$0$};
  \draw[{<[ipe arrow tiny]}-]
    (132, 784)
     -- (100, 772);
  \filldraw[shift={(84, 763.999)}, xscale=1.0833, yscale=0.8333, fill=white]
    (0, 0) rectangle (48, -24);
  \node[ipe node]
     at (92, 752) {$B'$};
  \node[ipe node]
     at (64.762, 741.906) {$\ell$};
  \draw[ipe dash dotted]
    (60, 776) rectangle (140, 740);
  \node[ipe node]
     at (144, 788) {$B_1$};
  \fill[white]
    (165.316, 794.322) rectangle (233.284, 782.647);
  \node[ipe node, font=\small]
     at (168.077, 786.857) {$\refB(B) \ldots \refB(B')$};
\end{tikzpicture}


==> pics/byz-equviocating.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \node[ipe node]
     at (44, 788) {$s$};
  \node[ipe node]
     at (44, 760) {$\byz{s}$};
  \draw[{<[ipe arrow tiny]}-]
    (132, 796)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (140, 780)
     -- (132, 764);
  \draw[shift={(64, 799.999)}, xscale=1.0833, yscale=0.8333]
    (0, 0) rectangle (48, -24);
  \draw[shift={(132, 799.999)}, xscale=1.0833, yscale=0.8333]
    (0, 0) rectangle (48, -24);
  \node[ipe node]
     at (68, 760) {$B$};
  \draw[shift={(64, 771.999)}, xscale=1.0833, yscale=0.8333]
    (0, 0) rectangle (48, -24);
  \node[ipe node]
     at (148, 808) {$1$};
  \node[ipe node]
     at (80, 808) {$0$};
  \draw[{<[ipe arrow tiny]}-]
    (100, 780)
     -- (100, 772);
  \filldraw[shift={(84, 763.999)}, xscale=1.0833, yscale=0.8333, fill=white]
    (0, 0) rectangle (48, -24);
  \node[ipe node]
     at (92, 752) {$B'$};
  \node[ipe node]
     at (64.762, 741.906) {$\ell$};
  \draw[ipe dash dotted]
    (60, 776) rectangle (140, 740);
  \node[ipe node]
     at (76, 788) {$B_1$};
  \node[ipe node]
     at (144, 788) {$B_2$};
\end{tikzpicture}


==> pics/intro.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \node[ipe node]
     at (64, 784) {$s_1$};
  \node[ipe node]
     at (64, 756) {$s_2$};
  \draw
    (88, 792) rectangle (112, 776);
  \draw
    (88, 764) rectangle (112, 748);
  \draw
    (88, 736) rectangle (112, 720);
  \draw
    (88, 708) rectangle (112, 692);
  \node[ipe node]
     at (64, 728) {$s_3$};
  \node[ipe node]
     at (64, 700) {$s_4$};
  \draw
    (128, 792) rectangle (152, 776);
  \draw
    (128, 764) rectangle (152, 748);
  \draw
    (128, 736) rectangle (152, 720);
  \draw
    (128, 708) rectangle (152, 692);
  \draw
    (168, 792) rectangle (192, 776);
  \draw
    (168, 764) rectangle (192, 748);
  \draw
    (168, 708) rectangle (192, 692);
  \draw
    (208, 792) rectangle (232, 776);
  \node[ipe node]
     at (96, 800) {$k_1$};
  \node[ipe node]
     at (132, 800) {$k_2$};
  \node[ipe node]
     at (172, 800) {$k_3$};
  \node[ipe node]
     at (212, 800) {$k_4$};
  \draw[{<[ipe arrow tiny]}-]
    (128, 788)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (168, 788)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (208, 788)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (128, 764)
     -- (112, 776);
  \draw[{<[ipe arrow tiny]}-]
    (128, 732)
     -- (112, 776);
  \draw[{<[ipe arrow tiny]}-]
    (128, 704)
     -- (112, 776);
  \draw[{<[ipe arrow tiny]}-]
    (168, 760)
     -- (152, 736);
  \filldraw[fill=white]
    (172, 704) rectangle (196, 688);
  \draw[{<[ipe arrow tiny]}-]
    (168, 760)
     -- (152, 704);
  \draw[{<[ipe arrow tiny]}-]
    (168, 760)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[shift={(48, 816)}, xscale=0.875, yscale=0.9524, gray]
    (0, 0) rectangle (224, -160);
  \draw[{<[ipe arrow tiny]}-]
    (128, 764)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (128, 736)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (128, 708)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (168, 708)
     arc[start angle=36.8699, end angle=143.1301, radius=10];
  \draw[{<[ipe arrow tiny]}-]
    (172, 700)
     arc[start angle=36.8699, end angle=143.1301, x radius=12.5, y radius=10];
  \node[ipe node]
     at (260, 784) {$s_1$};
  \node[ipe node]
     at (260, 756) {$s_2$};
  \draw
    (284, 792) rectangle (308, 776);
  \draw
    (284, 764) rectangle (308, 748);
  \draw
    (284, 736) rectangle (308, 720);
  \draw
    (284, 708) rectangle (308, 692);
  \node[ipe node]
     at (260, 728) {$s_3$};
  \node[ipe node]
     at (260, 700) {$s_4$};
  \draw
    (324, 792) rectangle (348, 776);
  \draw
    (324, 764) rectangle (348, 748);
  \draw
    (324, 736) rectangle (348, 720);
  \draw
    (324, 708) rectangle (348, 692);
  \draw
    (364, 792) rectangle (388, 776);
  \draw
    (364, 764) rectangle (388, 748);
  \draw
    (364, 708) rectangle (388, 692);
  \draw
    (404, 792) rectangle (428, 776);
  \node[ipe node]
     at (292, 800) {$k_1$};
  \node[ipe node]
     at (328, 800) {$k_2$};
  \node[ipe node]
     at (368, 800) {$k_3$};
  \node[ipe node]
     at (408, 800) {$k_4$};
  \draw[shift={(280, 796.001)}, xscale=0.6667, yscale=1.2308, line width=0.2, ipe dash dashed]
    (0, 0) rectangle (48, -104);
  \node[ipe node, font=\Large]
     at (292, 676) {$\mathcal{I}$};
  \node[ipe node, font=\Large, text=seagreen]
     at (300, 700) {\checkmark};
  \node[ipe node, font=\Large, text=seagreen]
     at (300, 728) {\checkmark};
  \node[ipe node, font=\Large, text=seagreen]
     at (300, 756) {\checkmark};
  \node[ipe node, font=\Large, text=seagreen]
     at (300, 784) {\checkmark};
  \draw[shift={(244, 816)}, xscale=0.8929, yscale=0.9512, gray]
    (0, 0) rectangle (224, -160);
  \filldraw[fill=white]
    (368, 704) rectangle (392, 688);
\end{tikzpicture}


==> tikzlibraryipe.code.tex <==

% Copyright (C) 2016  Joseph Rabinoff

% ipe2tikz is free software; you can redistribute it and/or modify it under
% the terms of the GNU General Public License as published by the Free
% Software Foundation; either version 3 of the License, or (at your option)
% any later version.

% ipe2tikz is distributed in the hope that it will be useful, but WITHOUT ANY
% WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the GNU General Public License for more
% details.

% You should have received a copy of the GNU General Public License along with
% ipe2tikz; if not, you can find it at "http://www.gnu.org/copyleft/gpl.html",
% or write to the Free Software Foundation, Inc., 675 Mass Ave, Cambridge, MA
% 02139, USA.


% ipe compatibility TikZ styles

\usetikzlibrary{arrows.meta}

\makeatletter

% These should behave almost exactly like ipe arrows.  They disable correcting
% for the miter length and line width.  This is important for visual consistency
% with ipe, since ipe arrows get much larger when the line width is increased.
% They also use the line join and cap styles from the main path.  These are very
% simple arrows: there is no harpoon version, and the convex hull computation is
% sloppy.

\pgfdeclarearrow{
  name = ipe _linear,
  defaults = {
    length = +1bp,
    width  = +.666bp,
    line width = +0pt 1,
  },
  setup code = {
    % Control points
    \pgfarrowssetbackend{0pt}
    \pgfarrowssetvisualbackend{
      \pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \pgfarrowssetlineend{\pgfarrowlength}
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % Convex hull
    \pgfarrowshullpoint{\pgfarrowlength}{0pt}
    \pgfarrowsupperhullpoint{0pt}{.5\pgfarrowwidth}
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth}}
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
  },
}


\pgfdeclarearrow{
  name = ipe _pointed,
  defaults = {
    length = +1bp,
    width  = +.666bp,
    inset  = +.2bp,
    line width = +0pt 1,
  },
  setup code = {
    % Control points
    \pgfarrowssetbackend{0pt}
    \pgfarrowssetvisualbackend{\pgfarrowinset}
    \pgfarrowssetlineend{\pgfarrowinset}
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % Convex hull
    \pgfarrowshullpoint{\pgfarrowlength}{0pt}
    \pgfarrowsupperhullpoint{0pt}{.5\pgfarrowwidth}
    \pgfarrowshullpoint{\pgfarrowinset}{0pt}
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowinset
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowinset}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth}}
    \pgfpathclose
    \ifpgfarrowopen
      \pgfusepathqstroke
    \else
      \ifdim\pgfarrowlinewidth>0pt\pgfusepathqfillstroke\else\pgfusepathqfill\fi
    \fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \the\pgfarrowinset,%
    \ifpgfarrowopen o\fi%
  },
}


% For correcting minipage width in stretched nodes
\newdimen\ipeminipagewidth
\def\ipestretchwidth#1{%
  \pgfmathsetlength{\ipeminipagewidth}{#1/\ipenodestretch}}

\tikzstyle{ipe import} = [
  % General ipe defaults
  x=1bp, y=1bp,
%
  % Nodes
  ipe node stretch/.store in=\ipenodestretch,
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe node/.style={
    anchor=base west, inner sep=0, outer sep=0, scale=\ipenodestretch
  },
%
  % Use a special key for the mark scale, so that the default can be overriden.
  % (This doesn't happen with the scale= key; those accumulate.)
  ipe mark scale/.store in=\ipemarkscale,
%
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
%
  ipe mark normal, % Set default
%
  ipe circle/.pic={
    \draw[line width=0.2*\ipemarkscale]
      (0,0) circle[radius=0.5*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe disk/.pic={
    \fill (0,0) circle[radius=0.6*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe fdisk/.pic={
    \filldraw[line width=0.2*\ipemarkscale]
      (0,0) circle[radius=0.5*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe box/.pic={
    \draw[line width=0.2*\ipemarkscale, line join=miter]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) rectangle
      ( .5*\ipemarkscale, .5*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe square/.pic={
    \fill
      (-.6*\ipemarkscale,-.6*\ipemarkscale) rectangle
      ( .6*\ipemarkscale, .6*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe fsquare/.pic={
    \filldraw[line width=0.2*\ipemarkscale, line join=miter]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) rectangle
      ( .5*\ipemarkscale, .5*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe cross/.pic={
    \draw[line width=0.2*\ipemarkscale, line cap=butt]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) --
      ( .5*\ipemarkscale, .5*\ipemarkscale)
      (-.5*\ipemarkscale, .5*\ipemarkscale) --
      ( .5*\ipemarkscale,-.5*\ipemarkscale);
    \coordinate () at (0,0);
  },
%
  % Arrow sizes (for TikZ arrows)
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=1},
  ipe arrow tiny/.style={scale=.4},
  ipe arrow small/.style={scale=.7},
  ipe arrow large/.style={scale=1.4},
  ipe arrow normal,
  /tikz/.cd,
%
  % Approximations to ipe arrows
  % Put in a style to allow to reset default scale when "ipe arrow normal" is
  % changed.  I think this is the only way, since all the parameters to arrows
  % are expanded when the tip is declared.
  ipe arrows/.style={
    ipe normal/.tip={
      ipe _pointed[length=1bp, width=.666bp, inset=0bp,
                   quick, ipe arrow normal]},
    ipe pointed/.tip={
      ipe _pointed[length=1bp, width=.666bp, inset=0.2bp,
                   quick, ipe arrow normal]},
    ipe linear/.tip={
      ipe _linear[length = 1bp, width=.666bp,
                  ipe arrow normal, quick]},
    ipe fnormal/.tip={ipe normal[fill=white]},
    ipe fpointed/.tip={ipe pointed[fill=white]},
    ipe double/.tip={ipe normal[] ipe normal},
    ipe fdouble/.tip={ipe fnormal[] ipe fnormal},
    % These should maybe use [bend], but that often looks bad unless it's on an
    % actual arc.
    ipe arc/.tip={ipe normal},
    ipe farc/.tip={ipe fnormal},
    ipe ptarc/.tip={ipe pointed},
    ipe fptarc/.tip={ipe fpointed},
  },
  ipe arrows, % Set default sizes
]

% I'm not sure how to do this in a .style, since the #args get confused.
\tikzset{
  rgb color/.code args={#1=#2}{%
    \definecolor{tempcolor-#1}{rgb}{#2}%
    \tikzset{#1=tempcolor-#1}%
  },
}

\makeatother

\endinput

